AGS-Mesh: Adaptive Gaussian Splatting and Meshing with Geometric Priors for Indoor Room Reconstruction Using Smartphones

Geometric priors are often used to enhance 3D reconstruction. With many smartphones featuring low-resolution depth sensors and the prevalence of off-the-shelf monocular geometry estimators, incorporating geometric priors as regularization signals has become common in 3D vision tasks. However, the accuracy of depth estimates from mobile devices is typically poor for highly detailed geometry, and monocular estimators often suffer from poor multi-view consistency and precision. In this work, we propose an approach for joint surface depth and normal refinement of Gaussian Splatting methods for accurate 3D reconstruction of indoor scenes. We develop supervision strategies that adaptively filters low-quality depth and normal estimates by comparing the consistency of the priors during optimization. We mitigate regularization in regions where prior estimates have high uncertainty or ambiguities. Our filtering strategy and optimization design demonstrate significant improvements in both mesh estimation and novel-view synthesis for both 3D and 2D Gaussian Splatting-based methods on challenging indoor room datasets. Furthermore, we explore the use of alternative meshing strategies for finer geometry extraction. We develop a scale-aware meshing strategy inspired by TSDF and octree-based isosurface extraction, which recovers finer details from Gaussian models compared to other commonly used open-source meshing tools. Our code is released in https://xuqianren.github.io/ags_mesh_website/.

==> author-kit-3DV2025-v1/tables/scannetpp.tex <==
\begin{figure*}[h!]
\centering
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_mesh2.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_normal2.jpg}
\end{subfigure}
\hspace{-10pt} 
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_mesh2.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_normal2.jpg}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_mesh2.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_normal2.jpg}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_mesh2.jpg}
        \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_normal2.jpg}
    \end{subfigure}
     \hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_mesh2.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_normal2.jpg}
\end{subfigure}
\\ %
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_mesh.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_normal.jpg}
    \subcaption{Reference}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_mesh.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_normal.jpg}
    \subcaption{Splatfacto}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_mesh.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_normal.jpg}
    \subcaption{Splatfacto + Ours}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_normal.jpg}
    \subcaption{2DGS}
\end{subfigure}
\hspace{-10pt}   
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our.jpg}
    \includegraphics[width=0.45\textwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_normal.jpg}
    \subcaption{2DGS + Ours}
\end{subfigure}
\caption{\textbf{Qualitative mesh comparison} for the "8b5caf3398" scene from ScanNet++ dataset.}
\label{fig:scannetpp-cmp}
\end{figure*}


==> author-kit-3DV2025-v1/tables/supp_mesh_figs.tex <==
\newcommand*\rot{\rotatebox{90}}
\newcommand{\fourwidth}{0.236\textwidth}

\begin{figure*}[t!]
    \centering
    \setlength{\tabcolsep}{0.1em}
    \renewcommand{\arraystretch}{0.8}
    \hfill{}\hspace*{-0.5em}
    \footnotesize
    \begin{tabular}{ccccc}
            \rot{\qquad\qquad\quad Reference}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_mesh2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_normal2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_mesh.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/gt_normal.jpg}
            \\
            \rot{\qquad\qquad Splatfacto~\cite{nerfstudio}}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_mesh2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_normal2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_mesh.jpg}& \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_normal.jpg}
            \\
            \rot{\qquad DN-Splatter~\cite{turkulainen2024dn} + Ours}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_mesh2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_normal2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_mesh.jpg}& \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/splatfacto_our_normal.jpg}
            \\
            \rot{\qquad\qquad 2DGS~\cite{Huang2DGS2024}}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_mesh2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_normal2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs.jpg}& \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_normal.jpg}
            \\
            \rot{\qquad\qquad 2DGS~\cite{Huang2DGS2024} + Ours}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_mesh2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_normal2.jpg}&
            \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our.jpg}& \includegraphics[width=\fourwidth]{author-kit-3DV2025-v1/Figures/figure4/2dgs_our_normal.jpg}
    \end{tabular}
  \caption{Qualitative mesh comparison for the "8b5caf3398" scene from ScanNet++ dataset.}
  \label{fig:scannetpp-cmp}
\end{figure*}
